Confidence Propagation through CNNs for Guided Sparse Depth Regression

Generally, convolutional neural networks (CNNs) process data on a regular grid, e.g. data generated by ordinary cameras. Designing CNNs for sparse and irregularly spaced input data is still an open research problem with numerous applications in autonomous driving, robotics, and surveillance. In this paper, we propose an algebraically-constrained normalized convolution layer for CNNs with highly sparse input that has a smaller number of network parameters compared to related work. We propose novel strategies for determining the confidence from the convolution operation and propagating it to consecutive layers. We also propose an objective function that simultaneously minimizes the data error while maximizing the output confidence. To integrate structural information, we also investigate fusion strategies to combine depth and RGB information in our normalized convolution network framework. In addition, we introduce the use of output confidence as an auxiliary information to improve the results. The capabilities of our normalized convolution network framework are demonstrated for the problem of scene depth completion. Comprehensive experiments are performed on the KITTI-Depth and the NYU-Depth-v2 datasets. The results clearly demonstrate that the proposed approach achieves superior performance while requiring only about 1-5% of the number of parameters compared to the state-of-the-art methods.

==> sec/method.tex <==
Here, we describe our approach by starting with a brief introduction to the normalized convolution framework. We then introduce an algebraically-constrained  normalized convolution operator for CNNs and the propagation method for confidences. Finally, we describe our proposed network architecture and the loss function taking confidences into account.

\subsection{Normalized Convolution}
Assume a sparse signal/image $\mathbf{F}$ with missing parts due to noise, acquisition process, preprocessing, or other system deficiencies. The missing parts of the signal are identified using a confidence mask $\mathbf{C}$, which has zeros or low values at missing/uncertain locations and ones otherwise. The signal is sampled and, at each sample point $k$, the neighborhood is represented as a finite dimensional vector $\mathbf{f}_k \in \mathbb{C}^n$ accompanied with a confidence vector $\mathbf{c}_k$ of the same size, both assumed to be column vectors. Using the notation from \cite{farneback:phd_thesis}, \emph{normalized convolution} is defined at all locations $k$ as (index $k$ is omitted to reduce clutter):
\begin{equation}\label{eq:1}
\mathbf{r} = (\mathbf{B}^* \mathbf{D}_\mathbf{a} \mathbf{D}_\mathbf{c} \mathbf{B})^{-1} \mathbf{B}^* \mathbf{D}_\mathbf{a} \mathbf{D}_\mathbf{c} \mathbf{f}\enspace,
\end{equation}
where $\mathbf{B}$ is a matrix which incorporates a set of basis functions $ \{ \mathbf{b}_i \in \C^n \}_1^m $ in its columns, $ \mathbf{D}_\times $ denotes a diagonal matrix with vectorized $\times$ on the diagonal, $\mathbf{a}$ is the applicability function which is a \emph{non-negative} localization function for the basis $\mathbf{B}$, and $\mathbf{r}$ holds the coefficients of the signal $\mathbf{F}$ at location $k$ projected onto the subspace spanned by $\mathbf{B}$.

The basis functions in $\mathbf{B}$ could be polynomials or complex exponentials, but the simplest case is when $\mathbf{B} = \{ \mathbf{b}_\mathbf{1}:\mathbf{b}_\mathbf{1} = \mathbf{1}\} $, and it becomes \emph{normalized averaging}. 
In this case, the signal is mapped onto a constant, localized with the applicability function, and (\ref{eq:1}) simplifies to %:
%\begin{equation}\label{eq:2}
$\mathbf{r} = (\mathbf{1}^* \mathbf{D}_\mathbf{a} \mathbf{D}_\mathbf{c} \mathbf{1})^{-1} \mathbf{1}^* \mathbf{D}_\mathbf{a} \mathbf{D}_\mathbf{c} \mathbf{f}$,
%\enspace,
%\end{equation}
which can be formulated for the full signal $\mathbf{F}$ and its confidence $\mathbf{C}$ as ($\ast$ denotes convolution and $\cdot$ point-wise multiplication):
\begin{equation} \label{eq:3}
	\mathbf{r}[k] = \dfrac{\sum_i \ \mathbf{a}[i] \  \mathbf{F}[k-i] \ \mathbf{C}[k-i]}{\sum_i \  \mathbf{a}[i] \ \mathbf{C}[k-i]} = \dfrac{\mathbf{a} \ast (\mathbf{F} \cdot \mathbf{C}) }{\mathbf{a} \ast \mathbf{C}} [k]\enspace,
\end{equation}

%-------------------------------------------------------------------------------

\subsection{Training the Applicability}
The appropriate choice of the applicability function is an open issue as it usually depends on the nature of the data. Therefore, methods for statically estimating the applicability function have been suggested %in the literature 
\cite{MM_SNA}, but we aim to learn $\mathbf{a}$ as part of the %network 
training. This generalizes convolutional layers, as normalized averaging is equivalent to standard convolution in case of signals with constant confidence.  As described above, the applicability function acts as a confidence or localization function for the basis and therefore it is essentially non-negative. 

Non-negative  applicabilities are feasible to train in standard frameworks,  since back-propagation is based on the chain rule and any differentiable function with non-negative co-domain can be plugged in. Thus, the function $\Gamma(\cdot)$, e.g. the softplus, is applied to the  the weights $\mathbf{W}$, and the gradients for the weight element $\mathbf{W}^l_{m,n}$ at the $l^\mathrm{th}$ convolution layer are calculated as:
\begin{equation}\label{eq:4}
\frac{\partial \mathbf{E}}{\partial \mathbf{W}^l_{m,n}} = \sum_{i,j} \frac{\partial \mathbf{E}}{\partial \mathbf{Z}^l_{i,j}} . \frac{\partial \mathbf{Z}^l_{i,j}}{\partial \ \Gamma (\mathbf{W}^l_{m,n})} . \frac{\partial \ \Gamma (\mathbf{W}^l_{m,n})}{\partial \mathbf{W}^l_{m,n}}\enspace,
\end{equation}
where $\mathbf{E}$ is the loss between the output and the ground truth,  $\mathbf{Z}^l_{i,j}$ is the output of the $\emph{l}^\mathrm{th}$ layer at locations $i,j$ that were convolved with the weight element $\mathbf{W}^l_{m,n}$. Accordingly, the forward pass for \emph{normalized convolution} is defined as:
\begin{equation}\label{eq:5}
\mathbf{Z}^l_{i,j} =  \frac{\sum_{m,n} \ \mathbf{Z}^{l-1}_{i+m,j+n} \mathbf{C}^{l-1}_{i+m,j+n} \ \Gamma (\mathbf{W}^l_{m,n})}{ \sum_{m,n} \ \mathbf{C}^{l-1}_{i+m,j+n} \ \Gamma(\mathbf{W}^l_{m,n}) + \epsilon}\enspace,
\end{equation}
where $\mathbf{C}^{l-1}$ is the confidence from the previous layer, $\mathbf{W}^l_{m,n}$ is the applicability in this context and $\epsilon$ is a constant to prevent division by zero. Note that this is formally a correlation, as it is a common notation in CNNs.

%-------------------------------------------------------------------------------

\subsection{Propagating Confidence}
The main strength about the signal/confidence philosophy is the availability of confidence information apart from the signal.  This is needed to be propagated through the network to output a pixel-wise confidence aside with the network prediction. In normalized convolution frameworks, Westelius \cite{Westelius302463} proposed a measure for propagating certainties:
\begin{equation}\label{eq:6}
\mathbf{C}_\mathrm{out} = \Big( \frac{\det \ \mathbf{G} }{\det \ \mathbf{G}_0 } \Big)^{\frac{1}{m}}\enspace,
%\mathbf{C}_\mathrm{out} = ( \det \mathbf{G} /\det \mathbf{G}_0 )^{\frac{1}{m}}\enspace,
\end{equation}
where $\mathbf{G} = (\mathbf{B}^* \mathbf{D}_a \mathbf{D}_c \mathbf{B})$, $\mathbf{G}_0 = (\mathbf{B}^* \mathbf{D}_a \mathbf{B})$ and  $m$ is the number of basis functions. 

This measure calculates a geometric ratio between the Grammian matrix $\mathbf{G}$ in case of partial confidence and $\mathbf{G}_0$ in case of full confidence. Setting $\mathbf{B} = \{ \mathbf{b}_\mathbf{1}:\mathbf{b}_\mathbf{1} = \mathbf{1}\} $, i.e., $m=1$,
we can utilize the already-computed term in (\ref{eq:5}) to propagate the confidence as follows:
\begin{equation}
\mathbf{C}^l_{i,j} = \frac{ \sum_{m,n} \mathbf{C}^{l-1}_{i+m,j+n} \ \Gamma( \mathbf{W}^l_{m,n}) + \epsilon}{\sum_{m,n} \ \Gamma(\mathbf{W}^l_{m,n})}\enspace,
%\mathbf{C}^l_{i,j} = \big(\sum_{m,n} \mathbf{C}^{l-1}_{i+m,j+n} \ \Gamma( \mathbf{W}^l_{m,n}) + \epsilon\big)\big/\big(\sum_{m,n} \ \Gamma(\mathbf{W}^l_{m,n})\big)\enspace,
\end{equation}


%-------------------------------------------------------------------------------

\subsection{Loss Function}
For scene depth completion task, we usually aim to minimize a norm, \textit{e.g}. \emph{l1} or \emph{l2} norm, between the output from the network and the ground truth. In our proposed method, we use the Huber norm, which is a hybrid between the \emph{l1} and the \emph{l2} norm and it is defined as:
\begin{equation}
\|z- t\|_\mathrm{H} =
\begin{cases} 
0.5(z-t)^2 & |z-t| < 1 \\ 
|z-t|-0.5, & \text{otherwise}
\end{cases}
\end{equation}
The Huber norm helps preventing exploding gradients in case of highly sparse data, which stabilizes the convergence of the network.
Nonetheless, our aim is not only to minimize the error norm between the output and the groundtruth, but also to increase the confidence of the output data. Thus, we propose a new loss which has a data term \emph{and} a confidence term:
\begin{equation}
 \mathbf{E}_{i,j} = \|\mathbf{Z}^L_{i,j} - \mathbf{T}_{i,j} \|_\mathrm{H} \enspace, \qquad \tilde{\mathbf{E}}_{i,j} = \mathbf{E}_{i,j} - \frac{1}{p} \left[ \mathbf{C}^L_{i,j} - \mathbf{E}_{i,j} \mathbf{C}^L_{i,j} \right] \enspace,
\end{equation}
where $\mathbf{Z}^L_{i,j}$ is the data output from the final layer $L$, $\mathbf{C}^L_{i,j}$ is the corresponding confidence output, $\mathbf{T}_{i,j}$ is the ground truth, $p$ is the epoch number, and $\|\cdot\|_\mathrm{H}$ is the Huber norm. The main objective of the loss is to minimize the error of the data term and maximize the confidence of the output. Note that the third term in the loss prevents the confidence from growing indefinitely. We weight the confidence term using the reciprocal of the epoch number $p$ to prevent it from dominating the loss function when the data error starts to converge.

%-------------------------------------------------------------------------------
\begin{figure*}[tbp]
\centering
\includegraphics[width=\textwidth]{fig/arch.pdf}
\caption{Our proposed multi-scale architecture for the task of scene depth completion which utilizes normalized convolution layers. Downsampling is performed using max pooling on confidence maps and the indices of the pooled pixels are used to select the same pixels from the feature maps. Different scales are fused by upsampling the coarser scale and concatenate it with the finer scale. A normalized convolution layer is then used fuse the feature maps based on the confidence information. Finally, a 1 $\times$ 1 normalized convolution layer is used to merge different channels into one channel dense output and output confidence map. }
\label{fig:arch}
\end{figure*}

\subsection{Network Architecture}
Inspired by \cite{Ronneberger2015}, we propose a hierarchical multi-scale architecture that shares the same weights between different scales, which leads to a very compact network as shown in Figure \ref{fig:arch}. Downsampling is performed using max pooling on the confidences and similar to \cite{zeiler2014visualizing} we keep the indices of the pooled pixels, which are then used to select the same pixels from the feature maps, \emph{i.e.}, we keep the most confident feature map pixels. The downsampled confidences are divided by the Jacobian of the scaling to maintain absolute confidence levels. Scale fusion is performed by upsampling the coarser scale and concatenate it with the finer scale. We apply a normalized convolution operator on the concatenated feature map to allow the network to fuse different scales utilizing confidence information. 

%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------

